Analyzing the Performance of Smart Industry 4.0 Applications on Cloud Computing Systems

Cloud-based Deep Neural Network (DNN) applications that make latency-sensitive inference are becoming an indispensable part of Industry 4.0. Due to the multi-tenancy and resource heterogeneity, both inherent to the cloud computing environments, the inference time of DNN-based applications are stochastic. Such stochasticity, if not captured, can potentially lead to low Quality of Service (QoS) or even a disaster in critical sectors, such as Oil and Gas industry. To make Industry 4.0 robust, solution architects and researchers need to understand the behavior of DNN-based applications and capture the stochasticity exists in their inference times. Accordingly, in this study, we provide a descriptive analysis of the inference time from two perspectives. First, we perform an application-centric analysis and statistically model the execution time of four categorically different DNN applications on both Amazon and Chameleon clouds. Second, we take a resource-centric approach and analyze a rate-based metric in form of Million Instruction Per Second (MIPS) for heterogeneous machines in the cloud. This non-parametric modeling, achieved via Jackknife and Bootstrap re-sampling methods, provides the confidence interval of MIPS for heterogeneous cloud machines. The findings of this research can be helpful for researchers and cloud solution architects to develop solutions that are robust against the stochastic nature of the inference time of DNN applications in the cloud and can offer a higher QoS to their users and avoid unintended outcomes.

==> Archive/sec-background.tex <==

\section{Background}
\label{sec-background}
During the past few years, there has been several confidentiality threats against users' data not just from external attackers, but from Cloud providers' insiders\cite{,,}. Therefore, Cloud providers are not considered a secure environment, specially for the patients' sensitive data. In particular, one major threat can be processing of the patients' data on unauthorized Virtual Machines (VMs). Another attack can be maliciously modifying a VM to read or modify the results of processing on the patients' data. 

To address these security concerns and be able to utilize the ubiquitous processing power of the Cloud services, we have implemented a system that verifies the authenticity of the offered Cloud resources before deploying them. That is, we assure that the patient's data can be merely uploaded and processed on trusted and intact (\ie not tampered) VMs. 

Our solution is based on using remote attestation~\cite{} of the VMs. Remote attestation enables authorized users to detect any changes to the users' computer. Trusted Platform Modules (TPM)~\cite{} is a dedicated embeded microprocessor that facilitates remote attestation in current computer devices (\eg desktop, laptops, and servers). TPM creates a hash key summary (also termed a fingerprint) of the hardware and software stack that booted on a computer. Since each TPM chip has a unique and secret RSA key burnt in as it is produced, it is capable of performing platform authentication. A user process can use the TPM to authenticate the hardware and software stack on a computer.

TPMs have also been utilized on Cloud hosts to make the offered services more resilient to confidentiality threats. Utilizing TPMs can restrict the upload of patient's data to Cloud hosts whose fingerprints are trusted. This capability remotely attests if a Cloud host is using an intact hardware and virtualization platform, which is called a \emph{hypervisor} in the literature. 

However, the operation of the TPM can be extended to the VMs running within the hypervisor of a Cloud host. A TPM for VMs, which is called a \emph{vTPM}~\cite{ibm}, works transparently and allows the users and applications not just attest the platform of a Cloud host but extends the attestation to the software stack within the VMs. That is, using vTPM we can assure that the user data are only uploaded on trusted Cloud hosts and trusted VMs. Therefore, the confidentiality of the patient's data and the software running in a guest VM even in the presence of a malicious system administrator is guaranteed.

Figure~\ref{} shows the way vTPM has been installed within the Cloud host.

To utilize vTPM for our VMs, we considered a quad-core, TPM-enabled server with Ubuntu 12.4 as the Cloud host. We installed a Xen 4.3 hypervisor with XSM/Flask security framework enabled on that. After installing Xen, we installed and configured Dom0, which is a default VM created by Xen to manage user VMs (called user domain or DomU in Xen). We installed a customized Linux kernel 3.7.1 for Dom0 that supports vTPM. We complied and configured Linux kernel 3.7.9 as DomU, which is, in fact, the VM image and can be instantiated by the user to create several VMs on a Cloud host. 

Once we set up the platform for the Cloud host, we can set up the vTPM. For that purpose, we should first set up the vTPM Manager which is, in fact, a minimal VM that creates and manages vTPM instances. The vTPM Manager requires a minimal disk image to store its encrypted data. After successfully creating the vTPM Manager, vTPM instances can be created. Similar to the vTPM Manager, a vTPM instance is also a VM with a disk image. Finally, in the VM template of the guest VM, we associate the VM to a created vTPM. This enables the cloud user to attest the software stack on the VM before uploading and processing the patient's data.

==> Archive/sec-heuristics.tex <==
\section{Proposed Heuristics}\label{sec:heuristics}
The proposed resource allocation model functions based on predefined heuristics. We have used three different heuristics along side with our probabilistic model heuristic in this research work. The outline of the heuristics used in this paper are given below in brief manner.

\subsubsection{\textbf{Minimum Expected Completion Time (MECT)}}
MECT heuristic is one of the baseline approaches in the literature. The core concept of this heuristic is to minimize the expected completion time of each arriving task to make an allocation decision. This heuristic uses the ETC matrix to calculate the average expected completion time ($\delta$) for the arriving task in every local edge nodes. Then the heuristic selects the edge node which offers the minimum expected completion time and allocates the task to that particular compute node. 



%Looking at the ETC matrix for a task's average completion time in a particular edge node. Whichever edge node provide small/less completion time, gets selected as task's processing unit and task is transferred to that edge node. This heuristic ignores the communication delay.​ value. This heuristic also ignores communication delay.​ar compute node.
%\subsubsection{\textbf{Maximum Robustness with Probability (MRP)}}
%According to the Maximum Robustness with Probability heuristic, the load balancer allocates the arriving task considering its robustness across the edge nodes. The robustness of a task is defined as the probability of that specific task to meet its deadline in a particular edge node.

%At first, the load balancer calculates the probability of the arriving task to meet its deadline in receiving edge. After that, the deadline meeting probabilities in all the neighboring edges are calculated. These probabilities are the set of values which represent robustness of the arriving task across the local edge nodes. From this robustness set, the heuristic chooses the edge that provides the maximum value (the highest probability) and allocates the task to that edge node. 

%Though, the highest probability needs to be greater than zero in order to be allocated. If there is no probability higher than zero within the set than the task is dropped.

%As the heuristic only selects one edge node for the allocation, the situation when two or more edge nodes have the same highest probability needs to be considered. In such situation, the tie can be resolved by considering the sparsity of two concurrent distributions. The sparsity is found from the standard deviations of respective distributions.

\subsubsection{\textbf{Maximum Certainty with Computation (MCC)}}
This heuristic is used in our previous work(\cite{hussainrobust}) considering utilizing only one edge without federation. In this work we use the same scheme but utilize the edge federation. This heuristic calculate the difference between task's deadline and average completion time. Then the task is transferred to the edge node which provides larger value. The analogy of this difference value is that, a task will be completed before it's deadline with the ``certainty" of the difference value. Here robustness is considered in terms of this certainty value which ignores the communication overhead. 

\subsubsection{\textbf{Traditional Edge Cloud (TEC)}}
This is one of the baseline heuristic where tasks are send to edge nodes or cloud datacenter based on their urgency. Specifically urgent tasks are transferred to edge whereas non-urgent delay tolerant tasks are send to cloud datacenter. In this heuristic edge federation is not used. Instead resource allocation scheme choose edge device randomly to assign tasks.

==> Archive/sec-implementation.tex <==

\section{Implementation}
\label{sec-implementation}
During the past few years, there has been several confidentiality threats against users' data not just from external attackers, but from Cloud providers' insiders\cite{Tang12,amini14}. Therefore, Clouds are not considered a secure environment, specially for the patients' sensitive data. In particular, one major threat can be processing of the patients' data on unauthorized Virtual Machines (VMs). Another threat can be maliciously modifying a VM to read or modify the results of processing on the patients' data. 

To address these security threats and be able to utilize the ubiquitous processing power of the Cloud services, we have implemented a system that verifies the authenticity of the offered Cloud resources before deploying them. That is, we assure that the patient's data can be merely uploaded and processed on trusted and intact (\ie not tampered) VMs. 

Our solution is based on using remote attestation~\cite{Santos12} of the VMs. Remote attestation enables authorized users to detect any changes to the users' computers. Trusted Platform Module (TPM)~\cite{perez06} is a dedicated embeded microprocessor that facilitates remote attestation in most of current computer devices (\eg desktop, laptops, and servers). TPM creates a hash key summary (also termed a fingerprint) of the hardware and software stack that booted on a computer. Since each TPM chip has a unique and secret RSA key burnt in as it is produced, it is capable of performing platform authentication. A user process can use the TPM to authenticate the hardware and software stack on a computer.

TPMs have also been utilized on Cloud hosts to make the offered services resilient to confidentiality threats. Utilizing TPMs can restrict upload of the patient's data to Cloud hosts whose fingerprints are trusted. This capability remotely attests if a Cloud host is using an intact hardware and virtualization platform (also called a \emph{hypervisor}) or not. 

However, the operation of the TPM can be extended to the VMs running within the hypervisor of a Cloud host. A TPM for VMs, which is called a \emph{vTPM}~\cite{perez06}, works transparently and allows the users and applications not just attest the platform of a Cloud host but extends the attestation to the software stack within the VMs. That is, using vTPM we can assure that the user data are only uploaded on trusted Cloud hosts and trusted VMs. Therefore, the confidentiality of the patient's data and the software running in a guest VM even in the presence of a malicious system administrator is guaranteed.

Figure~\ref{Fig:impl} shows the way vTPM has been set up within a Cloud host in our implementation.
To utilize vTPM for our VMs, we considered a quad-core, TPM-enabled server with Ubuntu 12.4 as the Cloud host. We installed a Xen 4.3 hypervisor with XSM/Flask security framework enabled on that. After installing Xen, we installed and configured Dom0, which is a default VM created by Xen to manage user VMs (called domain user or DomU in Xen). We installed a customized Linux kernel 3.7.1 for Dom0 that supports vTPM. We complied and configured Linux kernel 3.7.9 as DomU, which is, in fact, the VM image and can be instantiated by the user to create several VMs on a Cloud host. 

\begin{figure}
  \centering
  \includegraphics[width=0.45\textwidth]{Figures/implementation}
  \caption{Architectural view of the implementation that enables remote attestation for the application within the Virtual Machines (VMs).}
  \label{Fig:impl}
%   \vspace{-0.2in}
\end{figure}
Once we set up the platform for the Cloud host, we can set up the vTPM. For that purpose, we should first set up the vTPM Manager which is a minimal VM that creates and manages vTPM instances. The vTPM Manager requires a minimal disk image to store its encrypted data. After successfully creating the vTPM Manager, vTPM instances can be created. Similar to the vTPM Manager, a vTPM instance is also a VM with a disk image. Finally, in the VM template of the guest VM, we associate the VM to a created vTPM. This enables the cloud user to attest the software stack on the VM before uploading and processing the patient's data.

==> Archive/sec-simulation.tex <==
\section{Experimental Setup/Simulation}\label{sec:simulation}
Yet to done.

==> Sources/executionTime.tex <==
\section{Stochastic Inference Execution Time}\label{exetime}
The inference execution time of DNN applications is influenced by various factors (\ie energy, input data size, processing unit) that reflects uncertainty. Even if, the execution machine instance and application model remains same, multiple run of inference operation shows stochasticity in observed execution time. Hence, to visualize the stochasticity in inference time, we plot thirty runs of oil spill detection application in each of the selected machine instances of two cloud platforms. Figure \ref{fig:stochasticoilaws} and \ref{fig:stochasticoilcham} represent the stochastic nature of inference execution time in each of the selected instances of AWS and Chameleon cloud respectively. 

In figure \ref{fig:stochasticoilaws} and \ref{fig:stochasticoilcham}, the x axis presents the inference time whereas y axis represents the execution number within each machine instance of AWS and Chameleon cloud respectively. From figure \ref{fig:stochasticoilaws} we find that, the presence of stochasticity in inference execution times of oil spill detection application not only across various machine instances of AWS but also within each individual machine. Similar pattern for chameleon cloud platform is observed in figure \ref{fig:stochasticoilcham}. The presence of stochasticity leads to uncertain inference execution time unless any pattern is identified in observed data. Therefore, performing a precise modeling of inference execution times of DNN applications is essential for resource manager to perform real-time scheduling or task allocation in cloud platforms. In accordance, this model can be transformed into a matrix data form that represent estimated pattern of inference execution times for various DNN application's.  

\begin{table*}[h!]
\centering
\scalebox{0.68}
{\begin{tabular}{|l|l|l|l|l|l|}
\hline
\multicolumn{6}{|c|}{\textbf{Execution Time distribution with Shapiro-Wilk Test in AWS Cloud}}                                                                                                                                                                                                                                                                                                                                      \\ \hline
\textbf{App Type} \textbackslash \textbf{VM Type} & \textbf{Memory Optimized }                                                        & \textbf{Machine Learning Optimized}                                               & \textbf{GPU}                                                                      & \textbf{General Purpose}                                                          & \textbf{Compute Optimized}                                                        \\ \hline
\textit{Fire Detection}                  & \begin{tabular}[c]{@{}l@{}}Not Gaussian \\ (P = 0.0001)\end{tabular}     & \begin{tabular}[c]{@{}l@{}}Not Gaussian \\ (P = 0.0007)\end{tabular}     & \begin{tabular}[c]{@{}l@{}}Not Gaussian \\ (P = 0.0332)\end{tabular}     & \begin{tabular}[c]{@{}l@{}}Not Gaussian \\ (P = 0.0098)\end{tabular}     & \begin{tabular}[c]{@{}l@{}}Gaussian \\ (P = 0.3095)\end{tabular}         \\ \hline
\textit{Human Activity Recognition}      & \begin{tabular}[c]{@{}l@{}}Not Gaussian\\ (P = 3.9143e-08)\end{tabular}  & \begin{tabular}[c]{@{}l@{}}Not Gaussian \\ (P = 2.2110e-07)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Not Gaussian \\ (P = 6.6401e-08)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Not Gaussian \\ (P = 8.3748e-09)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Not Gaussian \\ (P = 1.1276e-09)\end{tabular} \\ \hline
\textit{Oil Spill Detection}             & \begin{tabular}[c]{@{}l@{}}Gaussian \\ (P = 0.0551)\end{tabular}         & \begin{tabular}[c]{@{}l@{}}Gaussian \\ (P = 0.2073)\end{tabular}         & \begin{tabular}[c]{@{}l@{}}Not Gaussian \\ (P = 0.0004)\end{tabular}     & \begin{tabular}[c]{@{}l@{}}Not Gaussian \\ (P = 5.6747e-10)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Gaussian \\ (P = 0.1472)\end{tabular}         \\ \hline
\textit{Acoustic Impedance Estimation}              & \begin{tabular}[c]{@{}l@{}}Not Gaussian \\ (P = 7.3109e-07)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Gaussian \\ (P = 0.1199)\end{tabular}         & \begin{tabular}[c]{@{}l@{}}Gaussian \\ (P = 0.8555)\end{tabular}         & \begin{tabular}[c]{@{}l@{}}Gaussian \\ (P = 0.2422)\end{tabular}         & \begin{tabular}[c]{@{}l@{}}Not Gaussian \\ (P = 0.0434)\end{tabular}     \\ \hline
\end{tabular}}
\caption{The execution time distributions of different DNN applications in AWS cloud's various instances are identified with Shapiro-Wilk test}
\label{tab:awsShaprio}
\end{table*}

\begin{table*}[h!]
\centering
\scalebox{0.75} 
{\begin{tabular}{|l|l|l|l|l|}
\hline
\multicolumn{5}{|c|}{\textbf{Execution Time distribution with Shapiro-Wilk Test in Chemeleon}}                                    \\ \hline
\textbf{App Type} \textbackslash \textbf{VM Type} & \textbf{m1.xlarge}    & \textbf{m1.large}     & \textbf{m1.medium}    & \textbf{storage.medium} \\ \hline
\textit{Fire Detection}                  & Gaussian     & Gaussian     & Not Gaussian & Not Gaussian   \\ \hline
\textit{Human Activity Recognition}      & Not Gaussian & Not Gaussian & Gaussian     & Not Gaussian   \\ \hline
\textit{Oil Spill Detection}             & Gaussian     & Not Gaussian & N/A          & N/A            \\ \hline
\textit{Acoustic Impedance Estimation}               & Gaussian     & Gaussian     & Gaussian     & Gaussian       \\ \hline
\end{tabular}}
\caption{The execution time distributions of DNN applications in Chameleon instances are identified with Shapiro-Wilk test}
\label{tab:chamShap}
\end{table*}


